Verifiable Reasoning for LLM-based Generative Recommendation

Reasoning in Large Language Models (LLMs) has recently shown strong potential in enhancing generative recommendation through deep understanding of complex user preference. Existing approaches follow a {reason-then-recommend} paradigm, where LLMs perform step-by-step reasoning before item generation. However, this paradigm inevitably suffers from reasoning degradation (i.e., homogeneous or error-accumulated reasoning) due to the lack of intermediate verification, thus undermining the recommendation. To bridge this gap, we propose a novel \textbf{\textit{reason-verify-recommend}} paradigm, which interleaves reasoning with verification to provide reliable feedback, guiding the reasoning process toward more faithful user preference understanding. To enable effective verification, we establish two key principles for verifier design: 1) reliability ensures accurate evaluation of reasoning correctness and informative guidance generation; and 2) multi-dimensionality emphasizes comprehensive verification across multi-dimensional user preferences. Accordingly, we propose an effective implementation called VRec. It employs a mixture of verifiers to ensure multi-dimensionality, while leveraging a proxy prediction objective to pursue reliability. Experiments on four real-world datasets demonstrate that VRec substantially enhances recommendation effectiveness and scalability without compromising efficiency. The codes can be found at https://github.com/Linxyhaha/Verifiable-Rec.

==> figs/4_exp.tex <==
\section{Experiments}\label{sec:exp}
In this section, we conduct experiments to answer the following research questions:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{RQ1}: How does the VRec perform compared to the baselines?
%     \item \textbf{RQ2}: How do the different components of VRec (\ie multi-dimensional verifiers, personalized router) affect the performance?
%     \item \textbf{RQ3}: How does VRec perform when scaling up the reasoning steps and verifier sizes? 
%     \item \textbf{RQ4}: How is the computational overhead of the verification step, and how is the hyper-parameter sensitivity? 
% \end{itemize}
\textbf{RQ1}: How does the VRec perform compared to the baselines? 
\textbf{RQ2}: How do the different components of VRec (\ie multi-dimensional verifiers, personalized router, monotonicity regularization, and verifier pre-training) affect the performance? 
\textbf{RQ3}: How does VRec perform when scaling up the reasoning steps and verifiers? 
\textbf{RQ4}: How is the computational overhead of the verification step, and how is the hyper-parameter sensitivity? 

\subsection{Experimental Settings}

\subsubsection{\textbf{Datasets}}
We conduct experiments on four real-world datasets from diverse domains, including music, micro-videos, and books. 
Specifically, we adopt two widely used Amazon review datasets\footnote{\url{https://jmcauley.ucsd.edu/data/amazon/}.}, 
1) \textbf{CDs} and 2) \textbf{Instruments}, 
which cover user interactions on music albums and instrument products with rich textual meta information such as titles and categories. 
In addition, we use a micro-video dataset 3) \textbf{MicroLens}\footnote{\url{https://github.com/westlake-repl/MicroLens/.}}, which contains extensive user interactions and textual descriptions for micro-videos~\cite{ni2023content}. 
Furthermore, we adopt 4) \textbf{Goodreads}\footnote{\url{https://cseweb.ucsd.edu/~jmcauley/datasets/goodreads.html/.}}, a book recommendation dataset that provides user interactions on books, where each item is provided with a book title, descriptions, and categories. 
% For data preprocessing, 
% we follow previous studies~\cite{bao2023bi} to ensure quality by filtering out users with fewer than 10 interactions. 
For each dataset, we sort user interactions chronologically based on timestamps and split them into training, validation, and testing sets with a ratio of 8:1:1. 
For each training instance, following~\cite{bao2024decoding}, we constrain the maximum length of item sequence to 10. 
The statistics of the four datasets are summarized in Table~\ref{tab:dataset_statistics} of Appendix. 

\noindent$\bullet\quad$\textbf{Evaluation.} 
To evaluate the models, we adopt the widely used Recall@$K$ (R@$K$) and NDCG@$K$ (N@$K$)~\cite{wang2021denoising}, with $K=5$ and $10$ to assess the recommendation accuracy. 
% In addition, we test the average inference time costs (s) per sample to analyze the model efficiency. 



\begin{table*}[t]
\setlength{\abovecaptionskip}{0.05cm}
\setlength{\belowcaptionskip}{0.2cm}
\caption{Overall performance of VRec and baselines on four real-world datasets. The best results are in bold and the second-best results are underlined. $*$ implies the improvements of VRec over the best baseline results are statistically significant ($p$-value < 0.01) under one-sample t-tests.}
\setlength{\tabcolsep}{2mm}{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|cccc|cccc|cccc}
\toprule
 & \multicolumn{4}{c|}{\textbf{CDs}} & \multicolumn{4}{c|}{\textbf{MicroLens}} & \multicolumn{4}{c|}{\textbf{Goodreads}} & \multicolumn{4}{c}{\textbf{Instruments}} \\ \midrule
\textbf{Method} & \textbf{R@5} & \textbf{R@10} & \textbf{N@5} & \textbf{N@10} & \textbf{R@5} & \textbf{R@10} & \textbf{N@5} & \textbf{N@10} & \textbf{R@5} & \textbf{R@10} & \textbf{N@5} & \textbf{N@10} & \textbf{R@5} & \textbf{R@10} & \textbf{N@5} & \textbf{N@10} \\ \hline
\textbf{GRU4Rec} & 0.0481 & 0.0671 & 0.0365 & 0.0426 & 0.0036 & 0.0068 & 0.0021 & 0.0031 & 0.0190 & 0.0332 & 0.0117 & 0.0163 & 0.0766 & 0.0938 & 0.0553 & 0.0609 \\
\textbf{Caser} & 0.0549 & 0.0749 & 0.0403 & 0.0467 & 0.0036 & 0.0063 & 0.0020 & 0.0029 & 0.0214 & 0.0378 & 0.0131 & 0.0183 & 0.0775 & 0.0972 & 0.0544 & 0.0608 \\
\textbf{SASRec} & 0.0784 & 0.0984 & 0.0576 & 0.0641 & 0.0044 & 0.0069 & 0.0029 & 0.0037 & 0.0182 & 0.0316 & 0.0114 & 0.0157 & 0.0825 & 0.0972 & 0.0726 & 0.0772 \\ \midrule
\textbf{TIGER} & 0.0381 & 0.0555 & 0.0269 & 0.0325 & 0.0052 & 0.0075 & 0.0023 & 0.0030 & 0.0202 & 0.0384 & 0.0116 & 0.0175 & 0.0760 & 0.0945 & 0.0557 & 0.0616 \\
\textbf{LETTER} & 0.0417 & 0.0619 & 0.0285 & 0.0350 & 0.0053 & 0.0104 & 0.0028 & 0.0045 & 0.0215 & 0.0377 & 0.0134 & 0.0185 & 0.0707 & 0.1012 & 0.0483 & 0.0583 \\
\textbf{SETRec} & 0.0627 & 0.0942 & 0.0454 & 0.0553 & 0.0094 & 0.0129 & 0.0055 & 0.0066 & 0.0106 & 0.0174 & 0.0066 & 0.0088 & 0.0786 & 0.0864 & 0.0721 & 0.0746 \\
\textbf{D3} & 0.0747 & 0.0940 & 0.0596 & 0.0659 & 0.0076 & 0.0134 & 0.0057 & 0.0076 & 0.0328 & 0.0534 & 0.0218 & 0.0285 & 0.0996 & 0.1188 & 0.0853 & 0.0915 \\
\textbf{LatentR3} & 0.0801 & 0.0978 & 0.0645 & 0.0703 & 0.0089 & {\ul 0.0160} & 0.0065 & 0.0088 & 0.0349 & 0.0565 & 0.0231 & 0.0301 & 0.1022 & 0.1243 & 0.0881 & 0.0951 \\ \midrule
\cellcolor{gray!8}\textbf{VRec-1Step} & \cellcolor{gray!8}{\ul 0.0836} & \cellcolor{gray!8}{\ul 0.1070} & \cellcolor{gray!8}{\ul 0.0655} & \cellcolor{gray!8}{\ul 0.0730} & \cellcolor{gray!8}{\ul 0.0100} & \cellcolor{gray!8}0.0154 & \cellcolor{gray!8}{\ul 0.0076} & \cellcolor{gray!8}{\ul 0.0093} & \cellcolor{gray!8}{{\ul 0.0365}} & \cellcolor{gray!8}\textbf{{0.0593}} & \cellcolor{gray!8}{{\ul 0.0236}} & \cellcolor{gray!8}{{\ul 0.0310}} & \cellcolor{gray!8}{{\ul 0.1067}} & \cellcolor{gray!8}{\ul 0.1269} & \cellcolor{gray!8}{\ul 0.0911} & \cellcolor{gray!8}{\ul 0.0976} \\
\cellcolor{gray!18}\textbf{VRec} & \cellcolor{gray!18}\textbf{0.0963*} & \cellcolor{gray!18}\textbf{0.1213*} & \cellcolor{gray!18}\textbf{0.0782*} & \cellcolor{gray!18}\textbf{0.0862*} & \cellcolor{gray!18}\textbf{0.0121*} & \cellcolor{gray!18}\textbf{0.0235*} & \cellcolor{gray!18}\textbf{0.0085*} & 
\cellcolor{gray!18}\textbf{\textbf{0.0121*}} & \cellcolor{gray!18}\textbf{\textbf{0.0366*}} & 
\cellcolor{gray!18}{{\ul 0.0582*}} &
\cellcolor{gray!18}\textbf{\textbf{0.0242*}} &
\cellcolor{gray!18}\textbf{\textbf{0.0312*}} &
\cellcolor{gray!18}\textbf{0.1098*} &
\cellcolor{gray!18}\textbf{0.1301*} &
\cellcolor{gray!18}\textbf{0.0944*} &
\cellcolor{gray!18}\textbf{0.0997*} \\ \bottomrule
\end{tabular}
}}

\label{tab:overall_performance}
\end{table*}

\subsubsection{\textbf{Baselines}}
We compare VRec with various competitive baselines, including traditional discriminative models, LLM-based generative models, and the LLM reasoning-enhanced models. Specifically, 
1) \textbf{GRU4Rec}~\cite{hidasi2015session} employs the gated recurrent unit (GRU) to capture the item's sequential patterns. 
2) \textbf{Caser}~\cite{tang2018personalized} utilizes convolutional neural networks (CNNs) to capture both sequential patterns and general user preference. 
3) \textbf{SASRec}~\cite{kang2018self} is one of the most representative sequential model, which leverages the bi-directional self-attention mechanism to effectively model the complex user behavior. 
4) \textbf{TIGER} ~\cite{rajput2023recommender} is a representative generative recommendation method that employs an RQ-VAE with codebooks to represent each item with a sequence of external tokens. 
5) \textbf{LETTER}~\cite{wang2024learnable} is also a external-token-based method, which integrates both semantic and collaborative filtering signals into item identifier to achieve recommendation that captures the collaborative similarity of items. 
6) \textbf{SETRec}~\cite{lin2025order} is a recent method that introduces order-agnostic item identifiers to better model user preference across different dimensions. 
7) \textbf{D3}~\cite{bao2024decoding} utilizes the item title with human vocabulary to represent each item, and emphasizes the more important tokens with collaborative information to achieve reliable recommendations. 
8) \textbf{LatentR$^3$}~\cite{zhang2025reinforced} is a recent reasoning-enhanced LLM-based method, where LLM first reasons the user preference in the latent space via an additional attention module before generating the next item. 


\subsubsection{\textbf{Implementation Details.}} 
For traditional methods, we search the learning rate and weight decay in the range of $\{1e^{-3}, 1e^{-4}, 1e^{-5}\}$ and $\{1e^{-3},1e^{-4}, 1e^{-5}, 1e^{-6}\}$, respectively. 
For both LLM-based baselines and VRec, we instantiate them on Qwen2.5-1.5B~\cite{qwen2025qwen25technicalreport} and fine-tune the full LLM parameters with learning rate searched from $3e^{-4},5e^{-5}, 3e^{-5}$. 
For LatentR$^3$ and VRec, we search the reasoning step $m$ in $\{1,2,4,6,8,10\}$. 
The coefficient of verifier prediction loss $\beta$ and the strength of monotonicity regularization $\gamma$ are selected from $\{0.3, 0.5, 0.7, 1\}$ and $\{0.1, 0.3, 0.5, 0.7, 1, 1\}$, respectively. 
We implement VRec on a pre-trained LatentR$^3$ for all experiments. 
All experiments are conducted on eight NVIDIA A100-SXM4-80G GPUs. 
More implementation details are provided in Appendix~\ref{app:detailed_descriptions}.





\subsection{Overall Performance (RQ1)}\label{sec:overall_performance}
The performance of VRec and baselines are presented in Table~\ref{tab:overall_performance}, from which we can observe that:
\begin{itemize}[leftmargin=*]
    % 1. 传统模型里面，sasrec通常有比较好的performance，这是因为它引入了双层注意力机制，利用了transformer，去建模item与item之间的dependency. 这个带来了两个好处：1）能够利用transformer的结构来capture Long-term semantics；2）同时又能够利用双向attention来选择那些更相关和更informative的信息，来understand user preference. 
    \item In traditional models (GRU4Rec, Caser, SASRec), SASRec typically achieves strong performance because it incorporates a two-layer attention mechanism based on the self-attention~\cite{vaswani2017attention} to model dependencies between items. 
    This design brings two main advantages: 1) it leverages the Transformer structure to capture long-term semantic dependencies, and 2) it utilizes bidirectional attention to focus on the most relevant and informative interactions, thereby enhancing the understanding of user preferences for appropriate recommendations. 
    % 2. LLM-based generative模型，用自然文本的模型会比用codebook或者embedding的模型(TIGER, LETTER, and SETRec) 有更好的performance。这是reasonable的，因为当利用大模型的时候, 这种codebook-based的方法往往需要更多的数据来做adaptation。
    \item Among LLM-based generative models, those that utilize human vocabulary (D3 and LatentR3) outperform codebook- (TIGER and LETTER) or embedding-based approaches (SETRec). This is reasonable, as codebook-based methods employ external tokens that are not seen in the LLM pre-training. As such, they typically require substantial data to adapt effectively to the items indexed by the external tokens when scaled to LLMs with billion-scale parameters. Similar observations are also seen in~\cite{bao2024decoding,lin2025order}.
    % 3. LatentR3在所有baseline里面consistently 超过了其他的basleine。这说明了reasoning的effectiveness。他通过引入一个额外的attention module来专门做reasoning，通过强化学习的方式鼓励模型去生成有助于推荐正确的item。it is noted that LatentR3的performance通常在reasoning step为1的时候有最好的效果，这和我们preliminary的观测一样，他们论文也有相同的观测和结论。
    \item Across baselines, LatentR$^3$ consistently surpasses all other methods, demonstrating the effectiveness of the reason-then-recommend paradigm. 
    By introducing an additional attention module dedicated to reasoning and employing reinforcement learning, LatentR$^3$ is encouraged to generate useful reasoning embeddings that facilitates accurate recommendations. It is worth noting that the best performance of LatentR$^3$ occurs with only 1 reasoning step, indicating the lack of scalability on reasoning steps, (\cf analysis in Section~\ref{sec:preliminaries}). This observation is also aligned with the findings reported in~\cite{zhang2025reinforced}.
    % 4. VRec的performance在四个数据集上consistently yield promising results。Specifically, VRec-1Step在大部分情况下都超过了baseline的表现。This 验证了verifiable reasoning仅在一个step上面也是有效的（对于一个step仍然可以做evaluation和adjustment，更好的帮助模型去推理user preference）（superior performance of VRec-1Step compared to LatentR$3$). 另外，VRec, which 是最优的reasoning step，允许超过1，它的performance consistently在四个数据集上超过了所有的baseline。这进一步验证了verifiable reasoning在扩展reasoning step上的有效性（further analysis of scalability on reasoining steps are presented in Section~\ref{}). 
    \item 
    VRec consistently achieves promising performance across all datasets. 
    In particular, VRec-1Step surpasses baselines in most cases. 
    This is expected due to the incorporation of the verification step, where the verifier can externally evaluate and adjust potentially inaccurate reasoning steps.
    Notably, when extended to multiple steps, VRec attains the best overall performance, demonstrating the scalability and robustness of the verifiable reasoning paradigm. Further analyses of reasoning scalability and a case study on homogeneity alleviation are presented in Section~\ref{sec:reasoning_step_scalability} and Appendix~\ref{app:additiona_results}., respectively.  
    
\end{itemize}
    


\subsection{In-depth Analysis}

\begin{figure}[t]
% \vspace{-0.2cm}
\setlength{\abovecaptionskip}{0.02cm}
\setlength{\belowcaptionskip}{-0.3cm}
\centering
\includegraphics[width=0.75\linewidth]{figures/ablation.pdf}
\caption{Ablation study of VRec on CDs dataset.}
\label{fig:ablation}
\end{figure}

\subsubsection{\textbf{Ablation Study (RQ2)}}
To study the effectiveness of the verification step in VRec, we remove the verification step denoted as ``w/o Verifier''. Besides, to validate the effectiveness of diverse verifiers, we instantiate VRec with only a single verifier from the category and title dimension, denoted as ``Single V-C'' and ``Single V-T'', respectively. 
We also discard the personalized router (``w/o VP) and the monotonicity regularization (``w/o $\mathcal{L}_{m}$''), and remove the verifier pre-training stage (``w/o VP), to evaluate the influence of these components, separately. 

The results on CDs dataset\footnote{We report the ablation study and reasoning scalability on MicroLens in Appendix~\ref{app:additiona_results} and omit results for other datasets with similar observations to save space.} are presented in Figure~\ref{fig:ablation}, where we can find that 
1) removing the verifier that disables the verification step (\ie the LatentR$^3$) leads to a significant performance decline. 
This validates the necessity of incorporating verifier and demonstrates the superiority of the reason-verify-recommend paradigm. 
In addition, 2) employing a single verifier would limit the effectiveness of the verification step, which emphasizes the importance of multi-dimensional verifier to achieve more accurate verification. 
Meanwhile, the inferior performance of VRec without personalized router further indicates the importance of individual-specific verification. 
Furthermore, 
3) removing monotonicity regularization can hurt the performance. This is expected since it can penalize the reasoning that leads to weak preference alignment. 
Lastly,
4) directly training the verifier and LLM recommender jointly leads to inferior recommendation results, which is probably due to the potential conflicts between the task of verifier prediction and the next item prediction if the verifier is trained from scratch. 
This issue can be alleviated by incorporating the verifier pre-training stage, which can adapt verifiers to the user preference space that aligns better with recommendation objectives. 

\subsubsection{\textbf{Reasoning Step Scalability (RQ3)}}\label{sec:reasoning_step_scalability}

\begin{figure}[t]
% \vspace{-0.2cm}
\setlength{\abovecaptionskip}{0.02cm}
\setlength{\belowcaptionskip}{-0.3cm}
\centering
\includegraphics[width=0.8\linewidth]{figures/scalability_dual_axis.pdf}
\caption{Scalability of reasoning steps of VRec.}
\label{fig:reasoning_step_scalability}
\end{figure}
% \HQ{Color coding may seem indifferentiable (especially the two blue lines). Maybe change to dashed line? Circle and square markers also look similar. Change to triangle?}

To investigate the potential of the verifiable reasoning paradigm, we vary the reasoning steps $m$ from 0 to 10 and report the results in Figure~\ref{fig:reasoning_step_scalability}. From the results, we can observe that 
1) the recommendation performance gradually improves as the reasoning step increases. This highlights the importance of the verification for the intermediate reasoning, which potentially corrects the reasoning process that misaligns with the user preference. 
% Despite the promising test-time scalability of VRec, the performance improvements 趋向于平原，增幅越来越小。这个可能是因为monotonicity regularization 鼓励模型prediction certainty要越来越强。这个会随着reasoning step的增大而让verifier要达到的目标越来越难，从而导致后面的reasoning step难以有significant的提升。
Despite the promising test-time scalability of VRec, 2) the performance gains tend to plateau (from {6 to 10 reasoning steps}). This may be because the monotonicity regularization encourages increasing prediction certainty, making it progressively harder for the verifier to achieve more accurate preference alignment as the reasoning steps deepen, thereby limiting significant improvements in later stages. 

\begin{table}[t]
\setlength{\abovecaptionskip}{0.05cm}
\setlength{\belowcaptionskip}{0.2cm}
\caption{Performance comparison of VRec of different verifier dimensions on CDs dataset.}
\setlength{\tabcolsep}{2mm}{
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{1}{l}{\textbf{Recall@5}} & \multicolumn{1}{l}{\textbf{Recall@10}} & \multicolumn{1}{l}{\textbf{NDCG@5}} & \multicolumn{1}{l}{\textbf{NDCG@10}} \\ \midrule
\textbf{Category} & 0.0854 & 0.1074 & 0.0678 & 0.0749 \\
\textbf{Category + Title} & 0.0940 & 0.1168 & 0.0775 & 0.0848 \\
\cellcolor[HTML]{ECF4FF}\textbf{Category + Title + CF} & \cellcolor[HTML]{ECF4FF}0.0973 & \cellcolor[HTML]{ECF4FF}0.1223 & \cellcolor[HTML]{ECF4FF}0.0796 & \cellcolor[HTML]{ECF4FF}0.0877 \\ \bottomrule
\end{tabular}
}}
\label{tab:verifier_diversity}
\end{table}



\begin{figure}[t]
\vspace{-0.2cm}
\setlength{\abovecaptionskip}{0.02cm}
\setlength{\belowcaptionskip}{-0.3cm}
\centering
\includegraphics[width=0.48\textwidth]{figures/verifier_size_scalability.pdf}
\caption{Performance comparison of VRec with different verifier model sizes on CDs dataset.}
\label{fig:verifier_size_scalability}
\end{figure}
\subsubsection{\textbf{Verifier  Scalability (RQ3)}}\label{sec:verifier_size_scalability}
% number of verifiers
% verifier model size
In VRec, the key component is the mixture of verifiers, where the model capacity of verifier might also be an important factor for effective verifiable reasoning.  
We investigate the scalability of verifiers from two perspectives:
\begin{itemize}[leftmargin=*]
    \item \textit{Dimensions of verifiers}. 
    % 我们逐步增加verifier的个数，对应的维度分别是category, title, 以及collaborative signals，探究增加维度的影响. 
    % From the results in Table XX, 我们可以看到当逐步扩展verifier的评判维度的时候，performance会持续提升。Notably, semantics的提升相较于cf会提升的更大，这个可能是因为LLM的推理space主要集中在语义部分，而并不擅长CF的捕捉（类似的现象也在xxx中被观测到）
    We gradually increase the number of verifiers, corresponding to the category, title, and collaborative signals, to examine the effect of expanding verification dimensions. From the results in Table~\ref{tab:verifier_diversity}, performance consistently improves as the evaluation dimension broadens. Notably, the improvement from semantic dimensions is more substantial than that from collaborative features, likely because the reasoning space of LLMs is primarily semantic, making them less effective at capturing collaborative patterns. Similar observation has also been reported in prior work~\cite{zhang2025collm}. 
    \item \textit{Model size of verifiers}. 
    We instantiate the verifier with an MLP and enlarge the hidden dimensions and the hidden layers to explore the scalability of verifier size on recommendation performance. The results in Figure~\ref{fig:verifier_size_scalability} shows that 
    % modestly把verifier变宽或者变深，能够进一步提高verification的质量，从而让recommendation更准确。但是不断变宽或扩深并不需要，这是因为verifier在做的是high-level的prediction task，类别通常在20左右，不是复杂的reasoning task，这种粗粒度的判别式任务，不需要太复杂，否则反而会overfitting。
    modestly increasing the width or depth of the verifier enhances verification quality, leading to more accurate recommendations, \eg competitive performance for {3 layer with 2048 hidden dimension}. However, continuously enlarging the verifier is unnecessary, as it performs a group-level prediction task with a limited number of classes (around 20) rather than complex reasoning. Excessive model capacity may therefore introduce overfitting rather than further improvement. 
\end{itemize}

% \subsubsection{\textbf{Generalization Analysis}}
% % gemma 


\begin{table}[t]
\setlength{\abovecaptionskip}{0.05cm}
\setlength{\belowcaptionskip}{0.2cm}
\caption{Comparison of average inference time costs (per sample) between LLM reasoning with (``w/'') and without (``w/o'') verifier on CDs dataset. }
\setlength{\tabcolsep}{2mm}{
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Reasoning Step} & \textbf{1} & \textbf{2} & \textbf{4} & \textbf{6} & \textbf{8} & \textbf{10} \\ \midrule
\textbf{w/o Verifier} & 0.754s & 0.825s & 0.896s & 0.946s & 1.064s & 1.142s \\
\textbf{w/ Verifier} & 0.761s & 0.831s & 0.908s & 0.950s & 1.065s & 1.142s \\
\cellcolor{gray!18}\textbf{\% Time Overhead} & \cellcolor{gray!18}0.97\% & \cellcolor{gray!18}0.71\% & \cellcolor{gray!18}1.33\% & \cellcolor{gray!18}0.46\% & \cellcolor{gray!18}0.06\% & \cellcolor{gray!18}0.03\% \\ \bottomrule
\end{tabular}
}}
\label{tab:efficiency}
\end{table}

\subsubsection{\textbf{Verifier Efficiency Analysis (RQ4)}}\label{sec:efficiency_analysis}
% 0 step, with/ wo verifier 
% To empirically analyze the computational overhead of the verification step to facilitate real-world applications, we test the VRec with and without verification across different reasoning steps. 
% As shown in Figure~\ref{}, 
% incorporating the verification step introduces additional computational overhead as expected. 
% Nonetheless, the computational overhead is neglectable (XXX\% additional time costs on average) as the main time costs are from the LLM itself. 
% As such, we may adjust the reasoning steps to strike the trade-off between the recommendation performance and the time costs from the reasoning steps. 
To empirically assess the computational overhead introduced by the verification step and its practicality in real-world applications, we evaluate VRec with and without verification across different reasoning steps. As shown in Table~\ref{tab:efficiency}, incorporating verification introduces a modest increase in computational cost, as expected. However, the overhead remains negligible (an average of 0.59\% additional time costs), since the majority of the computation is dominated by the LLM backbone. 
As such, the reasoning steps can be flexibly adjusted to balance recommendation performance and inference efficiency, while still benefiting from the performance gains brought by verification.





\begin{figure}[t]
\vspace{-0.2cm}
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.15cm}
  \centering 
  \hspace{-0.105in}
  \subfigure{
  \includegraphics[height=1.4in]{figures/hp_beta.pdf}} 
  % \hspace{-0.105in}
  \subfigure{    
  \includegraphics[height=1.4in]{figures/hp_gamma.pdf}} 
\caption{Performance of VRec with different strength of verifier loss $\beta$ and monotonicity regularization $\gamma$.}
% \CLEAN\HQ{Shall we use different colors for NDCG and Recall (like Fig 6)? nit, $\beta$ and $\gamma$ in the caption seem to be in bold font. }
  \label{fig:hp_analysis}
  % \vspace{-0.3cm}
\end{figure}

\subsubsection{\textbf{Hyper-parameter Sensitivity (RQ4)}} 

% alpha - negative sample strength for verifier training
% beta - v_weight
% gamma - mono
% In VRec, we introduce two key hyper-parameters (\ie strength of verifier prediction task $\beta$ and strength of monotonicity regularization). 
We further analyze hyper-parameters of VRec to facilitate future applications. 
% \noindent$\bullet\quad$\textbf{Effect of ${\beta}$}. 
1) \textbf{Effect of ${\beta}$}. 
From Figure~\ref{fig:hp_analysis}(a), we can observe that the recommendation accuracy first climbs up and then falls as the $\beta$ varies from 0 to 1. 
The verifier needs to maintain sufficient prediction capability to provide effective guidance. 
However, an overly strong verifier may conflict with the recommendation objective, thereby weakening the overall recommendation accuracy. 
2) \textbf{Effect of ${\gamma}$}. 
% 持续提高，说明了有效性。然后这个monotonicity regularization越提高，它的作用越饱和但不会往下掉，这个是合理的。因为可能当提高到一定程度的时候，它的penalty就忽略了，反而就没有起到更多作用（因为它只要不超过0就行）
As shown in Figure~\ref{fig:hp_analysis}(b), increasing the coefficient $\gamma$ of the monotonicity regularization consistently improves performance, demonstrating its effectiveness in promoting stable reasoning refinement. When $\gamma$ becomes sufficiently large, the improvement gradually saturates without performance degradation. 
This is reasonable, as the regularization term only penalizes non-monotonic entropy changes; once the reasoning process becomes stable (\ie the penalty approaches zero), further increasing $\gamma$ yields diminishing influence on optimization. 


% \subsubsection{\textbf{Case Study}}





==> figs/5_related_work.tex <==
\section{Related Work}\label{sec:related_work}

\subsection{Reasoning for Recommendation}
% \noindent$\bullet\quad$\textbf{Reasoning for Recommendation}. 
% 讲reasoning很promising，core idea就是让模型在给出最终的recommendation之前多让模型做几次推理，这在传统和基于大语言模型的都有些许工作进行探索。
% 对于llm推荐来讲，主要分为两类，一类是explicit, 一类是implicit。对于explicit来说，大部分工作都集中在ctr而不是next item prediction。因为cot难以构建，所以explicit reasoning不好搞。并且还有inefficency的问题，这对llm来说更致命。
% 为了克服没有cot数据的困难以及缓解inefficiency的问题，latent reasoning成为了一种更promising的方式。
% 虽然这些早期探索都demonstrate了promise of reason4rec, 但是他们都面临了一个很critical的问题：unveiried reasoning， 这个可以导致homogenous reasoning以及error-accumulated reeasoning，极大的限制了reasoning的潜力。
% 因此我们这个工作bridge了这个gap，提出了一个新的reason-verify-generate的范式，为llm reasoning提供intermediate feedback, 作为每一步reasoning的指导，最终lead to appropriate recommendations.
Recent advances highlight the promise of integrating reasoning into recommendation models, where the model performs multiple intermediate reasoning steps before making a final recommendation~\citep{wang2024enhancingrecommendersystemslarge,zhao2025reasontorecommendusinginteractionofthoughtreasoning,xie2025recllmr1twostagetrainingparadigm,gu2025r4ecreasoningreflectionrefinement,xing2025reg4recreasoningenhancedgenerativemodel,huang2025agenticrecommendersystemsera}. In LLM-based recommendation, existing efforts can be broadly categorized into explicit and implicit reasoning. Explicit approaches typically rely on supervised chain-of-thought (CoT) reasoning and are mostly explored in click-through-rate or rating prediction rather than next-item generation~\citep{xi2024towards,STARec2025,fang2025reason4rec}. However, constructing CoT data is costly, and explicit reasoning often suffers from inefficiency, which poses significant challenges for large-scale LLM deployment. In contrast, implicit (latent) reasoning eliminates the need for annotated CoT data and offers better efficiency~\citep{tang2025thinkrecommendunleashinglatent}. Nevertheless, prior studies inevitably encounter unverified reasoning, which leads to homogeneous shortcut reasoning and error accumulation across steps, thereby limiting the effectiveness of reasoning-based recommendations. 
To bridge this gap, our work introduces a novel verifiable reasoning paradigm that provides intermediate feedback at each reasoning step, auditing the reasoning towards a more faithful user preference understanding, unlocking the potential of reasoning. 


\subsection{Verifiable LLM Reasoning}
% \noindent$\bullet\quad$\textbf{{Verifiable LLM Reasoning}}
% existing work of general verifiable LLM reasoning


% external verifier
% internal signals (such as entropy)

% Recent research has increasingly explored verifiable reasoning to enhance the reliability of LLMs. 
Verifiable LLM reasoning involves structuring the model's reasoning process so that each intermediate step can be checked for correctness.
Existing studies can be broadly categorized into two groups. 
One line of work explores external-verifier, which explicitly evaluates intermediate reasoning steps using dedicated modules or reward models~\cite{wang2024mathshepherdverifyreinforcellms,zhang2025generativeverifiersrewardmodeling,zhang2025lessonsdevelopingprocessreward,zheng2025processbenchidentifyingprocesserrors}. 
% provide step-level supervision to assess the correctness of each chain-of-thought (CoT) step, outperforming outcome-only training on reasoning benchmarks. 
Frameworks such as Self-Refine~\cite{madaan2023selfrefineiterativerefinementselffeedback}, CRITIC~\cite{wang2023drdtdynamicreflectiondivergent,zheng2025criticcotboostingreasoningabilities}, and Tree-of-Thoughts~\cite{yao2023treethoughtsdeliberateproblem} iteratively verify and refine reasoning trajectories through learned critics or search-based evaluators. 
In contrast, 2) internal-signal approaches derive reliability cues from the model's own outputs. Self-Consistency~\cite{wang2023selfconsistencyimproveschainthought,li2023makinglargelanguagemodels,Taubenfeld_2025} aggregates multiple reasoning samples to identify consistent outcomes, while confidence- and entropy-based measures~\citep{wang20258020rulehighentropyminority} quantify uncertainty and calibration. 
However, these methods rely on explicit reasoning traces (\eg textual CoT), making them inefficient and hard to generalize to latent reasoning scenarios in next item recommendation. 
In this work, we propose a general verifiable reasoning framework specifically for LLM-based recommendation that operates on latent reasoning embeddings, achieving step-by-step reasoning verification. 

% wo propose a general verifiable reasoning framework for LLM-based recommendation that operates on latent reasoning embeddings. This design preserves the benefits of verifiability while remaining efficient, scalable, and effective without requiring explicit step-level supervision.

% gap: they can have the explicit data, while recommendation is implicit, so it is difficult to do so

==> figs/6_conclusion.tex <==
\section{Conclusion}

In this work, we pointed out the crucial issue of existing reasoning-enhanced LLM-based recommendation, \ie unverified reasoning that can lead to reasoning degradation. 
We then proposed a novel reason-verify-recommend paradigm that introduces an additional verification step to provide reliable feedback guidance for the reasoning process. 
We then summarized two principles for the verifier design, \ie 1) reliable evaluation and guidance feedback, and 2) multi-dimensional verifications. 
Meeting the two principles, we proposed VRec, which employs a mixture of verifiers with a personalized router to ensure multi-dimensional verification. 
To achieve reliable verification, we formulated a group-level preference prediction task for verifiers and leveraged internal model signals (\ie entropy and weights) for verification. 
Empirical results demonstrated the effectiveness, efficiency, and scalability of VRec. 
% and entropy-based evaluation. further stabilized by monotonicity regularization. Extensive experiments on four real-world datasets demonstrate that VRec consistently improves recommendation accuracy, robustness, and scalability, effectively mitigating homogeneous and error-accumulated reasoning.

This work takes the initial attempt to explore verifications for LLM reasoning in next item recommendation, leaving several promising directions. 1) Extending our framework on explicit reasoning for other recommendation tasks, such as CTR or rating prediction, is worth exploring. 2) While efficient, it is important to improve the interpretability and controllability of the verifiable reasoning in latent space,
Third, the design of verifiers presents rich opportunities for exploration, such as developing more expressive architectures and better alignment objectives to strengthen preference modeling and human-aligned verification. 
